Contrastive Learning Improves Model Robustness Under Label Noise

Deep neural network-based classifiers trained with the categorical cross-entropy (CCE) loss are sensitive to label noise in the training data. One common type of method that can mitigate the impact of label noise can be viewed as supervised robust methods; one can simply replace the CCE loss with a loss that is robust to label noise, or re-weight training samples and down-weight those with higher loss values. Recently, another type of method using semi-supervised learning (SSL) has been proposed, which augments these supervised robust methods to exploit (possibly) noisy samples more effectively. Although supervised robust methods perform well across different data types, they have been shown to be inferior to the SSL methods on image classification tasks under label noise. Therefore, it remains to be seen that whether these supervised robust methods can also perform well if they can utilize the unlabeled samples more effectively. In this paper, we show that by initializing supervised robust methods using representations learned through contrastive learning leads to significantly improved performance under label noise. Surprisingly, even the simplest method (training a classifier with the CCE loss) can outperform the state-of-the-art SSL method by more than 50\% under high label noise when initialized with contrastive learning. Our implementation will be publicly available at {\url{https://github.com/arghosh/noisy_label_pretrain}}.

==> methods.tex <==
\section{Contrastive Learning}
Contrastive learning has emerged as \ml{maybe say a key? avoid pissing people off} the key method for self-supervised visual representation learning. We will use the SimCLR contrastive model \ml{inconsistent terminology - make sure you clearly state what simclr is and what contrastive learning is, and stick with it throughout; a model, or a method to learn a model? you say contrastive learning is a method in the previous sentence. now it's a contrastive model. that does not look good.} \cite{simclr,simclrv2} throughout the paper; however, other visual representation learning models (including other contrastive models) can also potentially improve robustness under label noise. The main idea in learning a contrastive model \ml{learning a contrastive model? or learn representations using a contrastive loss? you have to be more precise here - what is a contrastive model? make it clear!} is to maximize the similarity of two augmented views of the same data point using a contrastive loss. 
In particular, we use a base encoder $f(\cdot)$ (ResNet-50 in this paper) to encode samples \ml{what is a sample? you call it ``data point'' in the previous sentence...} ${\bx}_i$ to $\bh_i=f({\bx}_i)$, and two layer MLP $g(\cdot)$ as the projection head to project into $\bz_i=g(\bh_i)$. In a set of $2N$ examples \ml{now you call it ``example''. great :) super sloppy!} $\{{\bx}_i\}$, for each example ${\bx}_i$, there is one positive example ${\bx}_j$ \ml{this part reads: for each example, there is one positive example and one negative example. not good. this terminology is not consistent and a mess. you cannot use terms interchangeably - pick one and stick with it!} (another view of the same sample), and $2N-2$ negative examples $\{{\bx}_k\}_{k\neq i, j}$. The contrastive loss  for a pair of positive example $i$, $j$, is defined as,
\begin{equation*}
    l_{i,j}=-\log\frac{\exp{(\text{sim}(\bz_i,\bz_j)/\tau)}}{\sum_{k,k\neq i}\exp{(\text{sim}(\bz_i,\bz_k)/\tau)}},
\end{equation*}
where $\tau$ is the temperature parameter, and $\text{sim}(\bz_i,\bz_j)$ is the normalized cosine similarity $\frac{\bz_i^{\intercal}\bz_j}{||\bz_i||||\bz_j||}$. We use the same noisy dataset \ml{what is the dataset? you should clearly define what is an image, what is its label, and what is the noise? it's not label noise since you're talking about contrastive learning, so i think it's the noisy views that you create, right? people may get confused because this paper is about label noise. then you say throw away the labels, so do you also throw away the noise? super confusing.} (throwing away the labels) to learn the contrastive model for visual representations. The base encoder $f(\cdot)$ (the ResNet-50 \ml{the resnet-50 WHAT? again, you say resnet-50 above and the resnet-50 model here. inconsistent.}) is then used as the initializer when learning with label noise. \ml{clearly state what is the consequence of all this - learned visual representations, h! what you wrote here is technically correct but creates significant barriers for a reader to follow through. try to guide them and make their life easier. you may not they will appreciate your effort.}

\section{Robust Learning under Label Noise}
\ml{this could've helped a ton in the previous section!!!}
We represent a sample image using $(\bx_i,\by_i)$ where $\bx_i$ is the feature vector of the  $i^{\text{th}}$ image and $\by_i\in \{0,1\}^K$ is the class label vector with $K$ total classes \ml{wrong - feature vector is h, I think?}. We denote the classifier as $f(\bx; \bw)$ \ml{bad notation: you used f as your encoder before!} where $\bw$ is the classifier weights \ml{parameters? that would encapsulate weights and biases}. Generally, we minimize the risk on the training samples using CCE loss $\ell_{\ce}$ as,
\begin{align*}
\bw^{\ast} =\argmin_{\bw}  \sum_{i\in \train} \ell_{\ce}(\by_i, f(\bx_i;\bw))
\vspace{-0.2in}
\end{align*}
We do not propose any new methods for handling label noise. We take two representative methods, one from inherently robust methods, and one from noise cleansing methods to show that a pre-trained contrastive model can improve noise robustness \ml{noise robustness? is that a term? robustness under label noise sounds more accurate? noise robustness sounds like a property of noise, not a method.} for any method. 

\paragraph{Generalized Cross-Entropy Loss}
Training with CCE loss is sensitive to label noise; in \cite{ghosh2017}, authors show symmetric losses such as Mean Absolute Error (MAE) is robust to uniform label noise. However, MAE is difficult to optimize in modern DNN architecture (even with clean samples). There have been many attempts to alleviate this problem with loss functions that is easy to optimize with provable noise robustness guarantees. \ml{so here this motivation seems repetitive - you've discussed this in the related work section. here i would just say something like: we take a representative loss that is shown to be robust to label noise...}
We take a representative method, generalized cross-entropy loss, that allows to trade-off noise robustness \ml{same problem as before} with optimization easiness \ml{this sounds awkward... easiness lol} \cite{generalized-ce}. In particular \ml{in particular? you're not listing a bunch of things. this should be specifically}, the generalized cross-entropy loss $L_q$ is defined as, \ml{no need to add , before you break for an equation}
\begin{equation*}
    L_q(f(\bx;\bw),\by) = \frac{1-f_y(\bx;\bw)^q }{q}
    \vspace{-0.1in}
\end{equation*}
where $q\in (0,1]$ \ml{q is what? a variable? an algorithm parameter?} and $f_y(\cdot)$ is the probability for class $\by$. Using \ml{the! aaaaaaah} limit theorem \ml{i googled what this is. all i could find is this thing called the CENTRAL limit theorem.}, it can be shown that $L_q$ loss is equivalent to CCE loss when $q\rightarrow 0$ and is equivalent to \ml{aaaaah} MAE loss when $q=1$. 

\paragraph{Meta-Weight Network}
Another common paradigm is to detect, reweigh \ml{the rule for commas: a, b, and c. if it's just two things you don't need the ,} possibly corrupted \ml{corrupted how?} samples while training. Meta-learning-based methods have been particularly useful to learn a reweighting strategy that performs well on an unbiased \ml{bias against what? in a paper you should be consistent - don't just throw out the term that comes off the top of your head... be consistent!} validation dataset \cite{mwnet,robust-mwnet,l2rw,l2l-noise}. We will use \ml{aaaaah} Meta-Weight Network (MWNet) as the representative method from this group \ml{of what? you haven't referred to a group before}. 
MWNet learns an \ml{an?!} weighting function $\CW$ with parameter $\theta$ \cite{mwnet}. Using a set of (small number of) clean  validation samples, MWNet learns the optimal weighting function $\theta^{\ast}$ in a bilevel optimization problem \cite{bilevel}. \ml{the use of a full stop is weird here} \ml{huge problems these last 2 sentences. first, you said W is a function, but what is its input and output? second, optimal weighting function is not the same as thetastar (which is a set of parameter values). these things correspond to each other but are not the same!}
\begin{align*}
&\min_{\theta} \CL^{\text{val}}(\bw^{\ast}(\theta))\triangleq\sum_{j\in \text{val}} \ell_{\ce}\Big(f(\bx_j;\bw^{\ast}(\theta)),\by_j\Big)\mbox{ s.t.}\\
&\bw^{\ast}(\theta)\!=\!\argmin_{\bw}\! \sum_{i\in \train}\! \CW\Big(\ell_{\ce}(\cdot,\cdot);\theta\!\Big)
\!\ell_{\ce}(f(\bx_i;\bw),\by_i) \nonumber
\end{align*}\ml{s.t. goes to the 2nd line!} \ml{you do not define what train and val are - sloppy}
The objective \ml{confusing word choice. i think you mean our objective is to ..., but it could be confused with the optimization objective. why not just say our goal here is to ...?} is to optimize for weighting network parameters $\theta$ such that the optimum classifier from the inner objective $\bw^{\ast}(\theta)$ (learned using the weighting parameter $\theta$) maximizes performance on the outer level meta \ml{train, val, meta - very confusing. you need more explanations here.} objective \ml{performance on objective does not make sense. you can say maximize performance on a problem, or maximize an objective.} (validation performances \ml{performance is singular}). 
Similar to many optimization-based meta-learning approaches, the weighting function (base classifier in meta-learning setup) is optimized with one step SGD in the inner objective \cite{maml,bilevel,mwnet}. \ml{inner problem makes more sense i think - you have inner and outer problems, they each have their own objective, and you solve them by taking a GD step w.r.t. an objective... your use of these terms here can be improved.}






==> old_exp.tex <==

\begin{table*}[t]\centering
    \scalebox{0.64}{
    \begin{tabular}{ccc cccccccc| cccccccc}\toprule
 \multirow{ 3}{*}{Model} & \multirow{ 3}{*}{Arch} & \multirow{ 3}{*}{Initializer}    &  \multicolumn{8}{c|}{CIFAR-10} &  \multicolumn{8}{c}{CIFAR-100} \\
    \cline{4-19}
            & &  &Clean & $0.2$ &$0.4$ &$0.5$ &$0.6$& $0.8$ & $0.9$ & $0.95$&Clean   &  $0.2$ &  $0.4$ &$0.5$ &$0.6$ & $0.8$ & $0.9$ & $0.95$\\
    \cline{1-19}        
    CCE  \cite{dividemix}& PRN-18 & No &  \multirow{4}{*}{95.11} &86.8&- & 79.4&- & 62.9 & 42.7& -&  \multirow{4}{*}{74.4}  &62.0&-& 46.7&- & 19.9 & 10.1  &-\\
    MLNT \cite{l2l-noise,dividemix} & PRN-18 & No &  &92.9 &-& 89.3 &-& 77.4 & 58.7 &-  && 68.5&- &59.2&- & 42.4 & 19.5 & -\\
    F-Correction \cite{forward,dividemix} & PRN-18 &No& & 86.8 &-& 79.8 &-& 63.3 &42.9 & - && 61.5&- &46.6&- & 19.9 & 10.2\\
    M-Correction \cite{m-correction,dividemix}& PRN-18 &No & &94.0&- & 92.0 &-& 86.8 & 69.1 & - &&  73.9&- & 66.1&- & 48.2 & 24.3 &-\\
    \cline{2-19}
    Divide-Mix \cite{dividemix} & PRN-18 &No & {95.8}&  96.1 &-& 94.6 &-& 93.2 & 76 & -& {78.9}  &77.3 &-& 74.6 &-& 60.2 & 31.5 & -\\
    \cline{2-19}
    MWNet \cite{mwnet} &WRN-28-10 & No &95.60&- & 89.27&-& 84.07 & - &- & -& 79.95&-& 67.73 &-&58.75&- & -&- \\
    \cline{2-19}
    $L_{q}$ \cite{generalized-ce} & RN-34 & No &\multirow{2}{*}{93.34} &89.83 & 87.13 &-& 82.54 & 64.07& - & -&\multirow{2}{*}{76.76} &66.81 &61.77 &-&53.16& 29.16 &-&-\\
     ELR \cite{elr} & RN-34 & No &&92.12& 91.43 & &88.87 & 80.69& -& -&&74.68  &68.43 & -& 60.05 & 30.27 & -&-\\
    \midrule
      CCE & RN-50 & INet32 &  \multirow{3}{*}{96.52} & 92.37 & -& 91.56& - & 83.34 & 62.66 & 39.09 &\multirow{3}{*}{81.51} & 70.26 & -& 65.76& -& 54.33 & 38.9 & 20.59 \\
    $L_q$ & RN-50 & INet32 & & 94.07&- & 93.75&- & 90.56& 85.89 & 73.14 & & 77.22 &-& 69.87&- & 60.5 & 54.83 & 44.3\\
    MWNet & RN-50 & INet32& & 97.33 & -& 96.17 &-& 93.12 & 90.88 & 85.27 & & 82.85&-& 80.28 &-&71.29 & 58.21 & 44.62\\
    \midrule
    CCE & RN-50 & SimCLR & \multirow{3}{*}{94.59} & 93.29 & -& 91.96 & -& 88.75 & 82.9 & 66.07 & \multirow{3}{*}{75.36} & 71.98 & -& 67.89 &- &59.84& 52.11 & 39.57\\
    $L_q$ & RN-50 & SimCLR & & 94.02 &-& 92.94 &-&90.85 & 88.45 & 83.76 & & 73.33 & -&70.14 &-&63.26 &55.93 & 45.7 \\
    MWNet & RN-50 & SimCLR & & 93.88 &-& 92.92 &-&91.51 &90.19 & 87.23 & & 73.2 & -& 69.88 &-&64.05 & 57.6&44.91\\
      \bottomrule
        \end{tabular}
    }%
    \vspace{0.03cm}
    \caption{Classification accuracy on the CIFAR-10/CIFAR-100 datasets under uniform noises. The clean accuracy \ml{what is clean accuracy. like clean water? something the united nations will love to see?} for Preactivated ResNet-18 (PRN-18) on DivideMix is using the Mixup training strategy \cite{mixup}; \ml{horrible sentence - you say ``accuracy is using the xxx strategy...} for other methods, the clean accuracy is from \ml{the} standard ERM objective with the CCE loss. Best methods are in {\bf bold}. \ml{you don't want to bold methods, you want to bold best performance under each setting?}
    }
    \label{tab:sym}
\end{table*}


\begin{table*}[t]\centering
    \scalebox{0.75}{
    \begin{tabular}{ccc cccc| cccc}\toprule
 \multirow{ 3}{*}{Model} & \multirow{ 3}{*}{Arch} & \multirow{ 3}{*}{Initializer}    &  \multicolumn{4}{c|}{CIFAR-10} &  \multicolumn{4}{c}{CIFAR-100} \\
    \cline{4-11}
            & & &Clean&  $0.2$ &$0.3$ &$0.4$ &  Clean &$0.2$ &  $0.3$ &$0.4$ \\
    \cline{1-11}      
    CCE \cite{generalized-ce} & RN-34 & No   &\multirow{4}{*}{93.34} &88.59 & 86.14&  80.11&  \multirow{4}{*}{76.76}&  59.20& 51.40 & 42.74\\
    { F-correction\cite{forward,generalized-ce}} & RN-34& No & &90.35& 89.25 & 88.12 && 71.08& 70.76& 70.82\\
    $L_q$\cite{generalized-ce} & RN-34 &No& &89.33& 85.45 & 76.74& &66.59& 61.45& 47.22\\
    ELR \cite{elr} & RN-34 & No  & &93.28 & 92.70 & 90.35&  &74.20 & 74.02 & 73.73\\
    \cline{2-11}
    MWNet \cite{mwnet} & WRN-28-10 & No  & 95.60& &  & & 79.95 & &  & \\
    \midrule
      CCE & RN-50 & INet32 &\multirow{3}{*}{96.52} &92.93 & 91.78 & 90.22 & \multirow{3}{*}{81.51}& 69.76 & 62.41 & 52.4\\
    $L_q$ & RN-50 & INet32 & & 93.77 & 93.23 & 90.24 & & 71.63 & 67.29 & 59.29\\
    MWNet & RN-50 & INet32 & & 96.85 & 95.9 & 94.99 & & 80.74 & 77.36 & 72.93\\
    \midrule
    CCE & RN-50 & SimCLR & \multirow{3}{*}{94.59}& 93.3 & 92.13 & 88.38 & \multirow{3}{*}{75.36}& 69.63 & 63.91 & 54.28\\
    $L_q$ & RN-50 & SimCLR & & 93.54 & 92.69 & 90.27 & & 71.26 & 68.04 & 59.26\\
    MWNet & RN-50 & SimCLR & & 93.67 & 93.18 & 92.59 & & 72.17 & 69.86 & 64.92\\
      \bottomrule
        \end{tabular}
    }%
    \vspace{0.03cm}
    \caption{Classification accuracy on the CIFAR-10/CIFAR-100 datasets under asymmetric noises. 
    }
    \label{tab:asym}
\end{table*}
\begin{table}[t]\centering
    \scalebox{0.85}{
    \begin{tabular}{ccc}\toprule
Model & Initializer & Accuracy\\
\midrule
CCE \cite{dividemix} & ImageNet & 68.94 \\
F-Correction \cite{forward} & ImageNet & 69.84\\
MLNT \cite{l2l-noise} & ImageNet & 73.47\\
DivideMix \cite{dividemix} &ImageNet & 74.76\\
ELR \cite{elr}& Imagenet & 72.87\\
ELR+ \cite{elr}& ImageNet & 74.81\\
\midrule
CCE & SimCLR & 73.27\\
$L_q$ & SimCLR & 73.35\\
MAE & SimCLR & 73.36\\
      \bottomrule
        \end{tabular}
    }%
    \vspace{0.03cm}
    \caption{Classification accuracy on  the Clothing1M dataset. \ml{in what context?}
    }
    \label{tab:clothing}
\end{table}
\section{Experimental Results}
We follow the standard experimental setup used in prior work \cite{mwnet,generalized-ce}. We use ResNet-50 (RN-50) \cite{resnet} \ml{as what?}; for CIFAR datasets, we use \ml{adopt} the common practice of replacing the first conv \ml{short for what? just conv sounds weird - write out the full word or use a special font or something} layer of kernel size 7, stride 2 with a conv layer of kernel size 3 and stride 1 and removing the first max-pool operation in RN-50 \cite{simclr}. 

{\bf Datasets:} We keep a random 1000 training samples as the validation set for the CIFAR-10/CIFAR-100 dataset. For the remaining 49000 \ml{training?} samples, we synthetically generate label noise. We keep the test dataset clean and list performance on the test dataset. We apply \ml{start with an over view: we use xxx types of label noise: uniform, asymmetric, ... another problem is that uniform is not the exact opposite of asymmetric - call it symmetric or call the other non-uniform?} the uniform noise with probability $\{0,0.2,0.5, 0.8,0.9, 0.95\}$ where the true class is uniformly corrupted to any of the classes (including the true class). 
We also experiment with the typical asymmetric noise scenario. We apply the asymmetric noise with probability $\{0.2, 0.3, 0.4\}$  where the true class label is corrupted to \ml{changed to?} a similar class, following the exact same setup used in prior research \cite{generalized-ce,forward}; for CIFAR-10, the class mappings are TRUCK $\rightarrow$ AUTOMOBILE, BIRD $\rightarrow$ AIRPLANE, DEER $\rightarrow$ HORSE, CAT $\leftrightarrow$ DOG. For CIFAR-100, the class mappings are generated from the next circular class \ml{circular class - is this a standard term? doesn't sound too informative.} (where 100 classes are categorized into 20 groups of 5 classes). 
We also compare our methods on the large-scale Clothing1M dataset with real-world noisy labels \ml{tiny detail - parallel structure: you said ``we synthetically generate label noise''. make this ``label noise is generally by human labelers'' and previously ``label noise is generated synthetically'' is probably a quick fix.} on 1 million training samples \cite{xiao2015learning}. 

{\bf SimCLR Training:} For training \ml{to train} the base encoder $\hat{f}(\cdot)$ and the projection head $g(\cdot)$, we use a batch size of 1024 (1200) and run for 1000 (300) epochs  with \ml{the} LARS optimizer \cite{lars} on a single NVIDIA RTX8000 (12 NVIDIA M40) GPU(s) on the CIFAR-10/100 (Clothing-1M) datasets. We use a learning rate of 4 (1.4), perform warmup \ml{jargon - what does warmup mean?} for 0.5\% (1\%) of the total iterations, and employ the cosine annealing strategy \ml{jargon - what does this strategy do? i know these are standard but you should still write a bit more here.} for the CIFAR-10/100 (Clothing1M) datasets.

{\bf ImageNet Pre-training:} We also compare the SimCLR initialization against the RN-50 model pre-trained on the ImageNet dataset. For the Clothing1M dataset, we use a standard pre-trained RN-50 classifier. For the CIFAR datasets, we train a RN-50 classifier from scratch (with CIFAR changes in the first conv layer) on the ImageNet-$32\times32$ (INet32) dataset that achieves 43.67\% Top-1 validation accuracy \cite{imagenet32} similar to \cite{pretraining}. \ml{not clear what this similar to is referring to}

{\bf Methods:} We use the SimCLR RN-50 initializer for three methods: \ml{no the here since you're not calling it a method} standard ERM training with the CCE loss, ERM training with the generalized cross-entropy loss $L_q$  (q=0.5 or 0.66), and MWNet. The value of q is important only for larger \ml{``high rate'' sounds more common i think?} noise rates ($\geq 0.8$), where a large q (0.66) is difficult to optimize \ml{``is'' is bad - you don't optimize q. it's more like picking this value results in a (numerically) hard-to-solve optimization problem, right?}; however, for all other noise rates, a higher value of q performs better \ml{q does not perform better. it leads to better performance}. We fine-tune for 120 epochs on the CIFAR datasets with \ml{better bring up SGD first before writing about param values} a learning rate of 0.01, SGD optimizer with a momentum of 0.9, weight-decay of 0.0001, batch size of 100, and warmup cosine annealing strategy (warmup for 1\% of the total iterations). 
For other baseline methods, we use the results listed in their respective papers. Note, \ml{bad language} different prior works use different architectures; thus, we also list the test accuracy from training on clean samples with that architecture (and initialization). \ml{this somehow doesn't seem too clear to me but i dont know how to fix}
We list the average accuracy from five runs of noise generations. \ml{i dont think you generate the noise explicitly? might as well call it noisy label generation? but then what about clothing which is already noisy?}

For the Clothing1M dataset, we compare with \ml{what is ``we''? here you say compare with xxx loss, ..., zzz loss - this reads as if you proposed a loss. you'd better say we USE these losses?} the CCE loss, the $L_q$ loss (q=0.66), and the MAE loss. We use a batch size of 32, \ml{same problem as above} SGD optimizer with a momentum of 0.9, and an initial learning rate of 0.001. For each epoch, we randomly sample 4000 batches of training samples such that classes are balanced \ml{does randomly sample this many batches give you balanced classes? in what? training? or each epoch?}, similar to \cite{dividemix,elr}. We fine-tune for 60 epochs and reduce the learning rate by a factor of 2 after every 10 epochs.






\subsection{Results and Discussion}
Table~\ref{tab:sym} lists the \ml{no the!} test performance \ml{not test performance i think? it's classification performance on the test set} under uniform label noise on the CIFAR datasets. The CCE loss, the $L_q$ loss, and the MWNet method improve performance significantly with the SimCLR initializer \ml{in this sentence you say ``method improve performance''. does not sound good. why not xxx init improves performance for ...?}. Under 90\% label noise, the CCE loss has an accuracy of 42.7\% (10.1\%) with a random initializer and DivideMix has an accuracy of 93.2\% (31.5\%) on the CIFAR-10 (CIFAR-100) dataset. Under the same noise rate, the CCE loss with the SimCLR initializer has an accuracy of 82.9\% (52.11\%) on the CIFAR-10 (100) dataset which translates to a 9\% (65\%) gain compared to the state-of-the-art method DivideMix. Further \ml{something. moreover, something. furthermore, something.}, the MWNet method and the $L_q$ loss improve \ml{same problem as before, simclr improves them, not they improve} performance significantly compared to the CCE loss with the SimCLR initializer. We tried to learn the MWNet model and the method based on $L_q$ loss on 95\% uniform noise rate with the random initializer, but we could not optimize these models under such a high noise rate. However, with the SimCLR initializer, these methods perform significantly better than the state-of-the-art method. \ml{this comes out of the blue here - you're saying these other things would crash under label noise this high? if so, begin by saying ``under very high levels of label noise, ...''}


Table~\ref{tab:asym} lists the test performance \ml{same as above} under asymmetric label noise on the CIFAR datasets. Similar to the uniform noise, we observe that the SimCLR initializer improves \ml{see? now you say simclr improves xxx. sounds much smoother, eh?} model robustness under asymmetric label noise. However, supervised robust methods do not beat the prior-state-of-the-art method ELR \ml{have you defined this abbreviation?} for the asymmetric noise case.

Table~\ref{tab:clothing} lists the test performance on the Clothing1M dataset. Although the CCE loss, the $L_q$ loss, and the MAE loss do not outperform state-of-the-art methods with the SimCLR initializer, they perform remarkably well without any specialized procedures. \ml{dunno what spacialized procedures are. jargon.} 

\ml{i don't think i really get this ``transfer'' thing - you can maybe start the imagenet pre-training paragraph above by quickly summarizing why are we comparing against this here}
{\bf ImageNet pre-training vs.\ SimCLR training: } We also observe that RN-50 pre-trained on the ImageNet dataset also improves model robustness under label noise. Note, \ml{same problem} there is significant overlap in \ml{between} the classes of the ImageNet dataset and \ml{that of} the CIFAR datasets. On the CIFAR-100 dataset, the test accuracy significantly improves to \ml{something significantly improves to sounds weird. say xxx significantly improves accuracy to xxx.} 81.51\% from fine-tuning the RN-50 pre-trained model (on INet32) compared to $\sim75\%$ with a random or the SimCLR initializer. 
However, the SimCLR initializer does not depend on \ml{require?} such a significant transfer of knowledge \ml{``significant transfer of knowledge'' sounds awkward} from another larger dataset. Further, \ml{same problem as above} we observe that the drop in performance (w.r.t.\ the accuracy from the clean training samples) is significantly lower for the SimCLR initializer compared to the pre-trained initializer. The pre-trained INet32 initializer seems to help more on \ml{in a case} the asymmetric noise case; class overlap and label corruptions to a similar class might be a reason behind this \ml{this what?}. In contrast, in the Clothing1M dataset, only two of the classes (out of 14) are present in the ImageNet dataset.
Consequently, the CCE loss with the SimCLR initializer improves the test performance by 3.3 points \ml{like points on an exam?} compared to the ImageNet pre-trained RN-50 initializer. 

\section{Conclusion}
Supervised robust methods are especially susceptible to label noise \ml{the name is bad here - these methods have ``robust'' in their name, but susceptible to label noise - sounds weird.} on vision \ml{image?} datasets where representation learning is more important \ml{than what? when you dish out a comparison, you can just say A is more xx. you have to say A is more xx than B.}.
We have shown that many supervised robust methods perform significantly better with the SimCLR initializer. \ml{you should list the representation stuff here as a possible cause.}
Equipped with the SimCLR initializer, even the CCE loss can beat the state-of-the-art SSL method in some cases. Thus, we advocate using the CCE loss with the SimCLR initializer as the new baseline method for learning under label noise on vision datasets.
\ml{the next sentence sounds weird; this shouldn't belong here. i would just cut this if we need more space}
However, we do not advocate any specific earlier works; instead, we intend to show that these supervised robust methods performed inferior to the SSL methods due to the lack of learning visual representation. 
We believe extending our work to other supervised robust methods will enable many prior them \ml{many prior them?!} to be strong contenders to the SSL methods on vision datasets. Further, we believe decoupling the representation learning problem from the task of learning under label noise would bring new methods that can do well on either of these tasks while they may fail on the other task. \ml{idea is good but the writing can be improved - apply the same rules you learned from the intro here and the abstract!}

==> old_intro.tex <==

\section{Introduction}

\ml{main problem with your writing: you have too much jargon. can you guarantee everyone who reviews your paper is familiar with this line of work? no. so you should BRIEFLY explain what these things do instead of throwing out a term such as ``MixUp''. yes, i am an amateur on this topic, and many other topics, but i'm not stupid - from a reviewer's point of view, i would very much enjoy it if you can help me get a rough idea of what's going on in this area. then i can pick up the key idea and form a judgement. don't estimate people's ability to learn things they're not familiar with even from only reading a single WELL-WRITTEN paper.}

Deep neural networks (DNN), trained with \ml{not precise: you assume a lot of unsaid things here - label means the DNN is used for a classification task, where you minimize losses... making it a little bit more explicit helps.} categorical cross-entropy (CCE) loss, are sensitive to label noise. 
Several methods, often endowed with a robust loss functions, tackle label noise inherently \ml{i know what you mean by ``inherently'' after seeing your wacv paper. but it comes out of the blue here - what i would call jargon. you may get away with it in some situations but it's not good practice. here one easy thing you can do is - you say robust lost functions. robust to what? explaining it in a few words would work - that way you make it clear that the trick these methods do is to change the loss function itself.} \cite{generalized-ce,peer,normalized-loss,ghosh2015,ghosh2017-dt,ghosh2017,unhinged,peer,ldmi}. 
However, robust losses are sometimes difficult to optimize with \ml{``with'' is not precise. you optimize an objective with an algorithm such as SGD. you can say in conjunction with or explain a bit more, briefly summarizing your prior work...} DNNs \cite{generalized-ce}.
Thus, a group of methods also propose  noise-cleaning \ml{from what you described below these methods do not ``clean'' the noise - your text suggests that they find noisy samples and treat them differently. you're not killing the noise. is this a standard term?} modules to separate noisy samples in the standard training process with \ml{the} CCE loss \ml{``the'' has been a consistent problem - you need it here since CCE is a specific thing, just like you need it where you say ``the AUC metric'', ``the Adam optimizer'' - it's a special thing that is different from others.} \cite{mwnet,l2rw,robust-mwnet,cleannet,co-teaching,glc,l2l-noise,m-correction}. \ml{this is again ambiguous - i would imagine you say high loss samples are noisier ones - you can make that explicit by adding just a few more words.}
Recently, several methods propose a semi-supervised framework that leverages unlabeled samples in addition to the noise-cleaning modules \cite{dividemix,elr}. 
These models leverage the power of self-supervised learning to improve visual representation learning from the unlabeled samples; e.g., DivideMix uses MixUp \ml{here's a point where you're stuck in the middle - you should either make it more specific, i.e., say what does MixUP actually do, or cut the crap here. just throwing this out here is again jargon without proper context.} consistency regularization and \ml{again, you need the here since it's a specific strategy} entropy minimization strategy \cite{mixup,dividemix}.
These semi-supervised strategies have been highly successful compared to prior supervised robust learning methods \cite{dividemix}. \ml{``supervised robust learning methods'' - is that a standard term?}
Thus, it is natural to ask whether the significant performance drop \ml{inconsistent and imprecise language - go over what you wrote above again - you surveyed a bunch of methods, saying the last type (semi-supervised) is better. you don't talk about a ``drop''. I know you're referring to the first type underperforming the second type, but you have to use more consistent language - either say robust xxx suffers a drop in performanced compared to semi-supervised or say: is the improvement of semi-supervised over robust xxx is caused by robustness to label noise or good visual representations? the point is consistency - we see A<B, and why is A<B? you shouldn't say B>A, and then why is A<B.} of supervised robust methods is due to the \emph{sensitivity} to label noise or because of not able to learn a \emph{`good' visual representations} under label noise. \ml{A xx representationS - many such instances.}

\ml{from this point on, the organization is messed up. you start by overviewing methods to combat label noise, and the observation that in prior literature, semi-supervised methods win. that actually makes sense. however, from now on, i have no idea what is your contribution (this paragraph? it reads like a research diary), what is the related work discussion (next paragraph)? make it clear! the structure of the first part of a paper should be - background, motivation, contributions, related work. you should list things like contrastive learning in the motivation since your contribution statements need it - it can't come later. you should mention each method BRIEFLY, intuitively summarizing what it does.}
\ml{i always like to structure my paragraphs this way - 1. background + (maybe 2) what is an important problem, 2. how do people solve it - what is the problem with this approach/these approaches, 3. another way people solve it - repeat, ..., 4. what research questions do we ask from these observations or what is missing and needs to be done, 5. contributions - what is our approach to tackle which problem, briefly summarize our approach, how did we justify it, what are some possible takeaways, 6. related work - what do competitive/similar methods do, and how is it different compared to our approach. you seem to already do this last part in the last paragraph, but it needs to be structured better.}

\ml{let me give you an example of quickly summarizing something without going into details. say for contrastive learning. i'm not an expert there and don't know all the details. but here's a summary - ``contrastive learning uses a self-supervision pre-traing method to learn good visual representations of images through comparing and contrasting different versions of an original image under various common perturbations.'' not far off, huh?}

\ml{this half sentence lol} We find that although CCE loss is sensitive to label, as proved in prior research \cite{ghosh2017}, the significant portion of the performance drop when training with CCE loss, is because of a lack of learning good visual representations. 
In contrast, semi-supervised methods can effectively learn visual representations even under label noise improving their performances. 
Surprisingly, we find when initialized with a proper visual representation model, the CCE loss can beat other noise-robust models, including state-of-the-art methods (trained with random initializer) under severe label noise. 
However, the point is not to advocate the use of CCE loss under label noise; instead, we show many prior supervised noise-robust methods improve significantly when properly initialized. 
For example, generalized cross-entropy loss \cite{generalized-ce}, a robust loss, can retain good performance even under 95\% uniform label noise on the CIFAR-100 dataset whereas training with a random initializer does not perform better than a random model.
This observation brings another question on whether the current baseline methods should be learning the visual representations and the label noise problem altogether? 
We believe decoupling these two separate problems would bring new methods that can do very well on either of these tasks while they may fail on the other task. 

\ml{key writing tip: parallel structure. when you discuss several different things, keep a RIGID structure: First, xx method does xxx [], which ... As a result, it achieves xxx. However, it fails to xxx. Second, yy method does yyy [], which ... As a result, it achieves yyy... Each thing has to follow the same RIGID structure as much as possible. it would make things look super nice and very easy to follow.}
However, the idea of using a pre-trained model initializer or self-supervised learning is not new, even in the label noise research. 
In \cite{self-supervision}, authors use the auxiliary tasks, such as rotation prediction to improves robustness under label noise.
In \cite{pretraining}, authors use a pre-trained Imagenet model to improve robustness. 
In contrast, our work does not use any auxiliary task or use a pre-trained model from other datasets.
We use the same noisy dataset for training a contrastive model that initialize the network when learning with label noise.
Thus, datasets that have a significant covariate shift between pre-training datasets (most often ImageNet) can still be handled using the contrastive \ml{jargon - dropping it here without explaining what it is makes absolutely zero sense.} model initializer. 
The closest to our work is \cite{c2d}, which uses contrastive pre-trained models to improve the DivideMix algorithm. 
However, we show that a self-supervised contrastive model initializer can improve robustness under label noise for many supervised base models. 
In particular, training with sensitive cross-entropy loss (with contrastive initializer) can also beat state-of-the-art label noise methods. 
Moreover, we show for two specific methods (one noise-tolerant method, and one noise-cleaning method), used in literature, that they can offer significant improvement under label noise than cross-entropy loss with the right initializer. 
With the right initialization, robust supervised methods can concentrate on the main task of learning with label noise. 
Before delving into specific methods used in this paper, we provide background on contrastive representation learning.


\ml{key writing tip: put yourself into the reviewer's shoes. think about it from their angle. when you write something, read it again - does it follow from the previous sentence? does it build up to what you're going to write next? a paper should be coherent - you can't dump something in without motivating it or giving people enough to anticipate it. put it into the context of the paper - are all the terms clear and unambiguous? do they clearly refer to something?}



